Endogenizing Epistemic Actions

Through a series of examples, we illustrate some important drawbacks that the action logic framework suffers from in its ability to represent the dynamics of information updates. We argue that these problems stem from the fact that the action model, a central construct designed to encode agents' uncertainty about actions, is itself effectively common knowledge amongst the agents. In response to these difficulties, we motivate and propose an alternative semantics that avoids them by (roughly speaking) endogenizing the action model. We discuss the relationship to action logic, and provide a sound and complete axiomatization.

==> eptcsdata.tex <==
\providecommand{\firstpage}{426}
\providecommand{\publicationstatus}{J. Lang (Ed.): TARK 2017\\
EPTCS 251, 2017, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.251.31}{10.4204/EPTCS.251.31}}

